Putting It All into Context: Simplifying Agents with LCLMs

Recent advances in language model (LM) agents have demonstrated significant potential for automating complex real-world tasks. To make progress on these difficult tasks, LM agent architectures have become increasingly complex, often incorporating multi-step retrieval tools, multiple agents, and scaffolding adapted to the underlying LM. In this work, we investigate whether all of this complexity is necessary, or if parts of these scaffolds can be removed on challenging tasks like SWE-bench. We show that in the case of SWE-bench, simply putting the entire environment into the context of a long context language model (LCLM) and properly prompting the model makes it competitive with carefully tuned, complex agent scaffolds. We show that a Gemini-1.5-Pro model without any scaffolding or tools achieves 38% on SWE-Bench-Verified, comparable with approaches using carefully tuned agent scaffolds (32%). While the unscaffolded approach with Gemini-1.5-Pro falls short of the strongest agentic architectures, we demonstrate that the more capable Gemini-2.5-Pro using the same unscaffolded approach directly attains a 50.8% solve rate. Additionally, a two-stage approach combining Gemini-1.5-Pro with Claude-3.7 achieves a competitive 48.6% solve rate.

==> sections/intro_condensed.tex <==
 Language model (LM) agents have gained significant attention in demonstrating their ability to perform complex real-world tasks autonomously \citep{yao2023react,shen2023hugginggpt}. Specifically, in the recent past, LM agents have been explored for complex coding tasks such as fixing bugs in public github repositories~\citep{starcoder,wang2024executablecodeactionselicit,yang2024sweagentagentcomputerinterfacesenable}.  These approaches are primarily driven by the introduction of SWE-Bench, a dataset that evaluates the agent's ability to resolve github issues that involves gathering information by searching and navigating complex github repositories, reasoning to understand the dependencies between functions in multiple files, and taking actions to identify and fix the error in code~\citep{swebench}.  

\input{figures/main_illustration}

Two primary methodologies have been developed to address these tasks: agentic pipelines \citep{yang2024sweagentagentcomputerinterfacesenable, wang2024executablecodeactionselicit} and non-iterative scaffolding approaches \citep{xia2024agentlessdemystifyingllmbasedsoftware,ehrlich2025codemonkeysscalingtesttimecompute}. Agentic frameworks employ multi-turn interactions with tools such as file/code search and shell command execution to mimic human developers' workflows. Meanwhile, non-agentic methods like Agentless propose structured scaffolds for localization, repair candidate generation, and validation through testing. While these approaches demonstrate promising results, they share a common limitation: they rely heavily on carefully human-designed  scaffolding. The need for sophisticated scaffolding in previous methods stems from the challenging localization process, which forces LM to execute sequential operations to obtain accurate, yet still partial, observations without complete state visibility. 

%Typically, LM agents interact with the environment to gather information, reason, and then execute actions based on this information to achieve predefined objectives. While information gathering forms the foundation of these system -- and researchers develop frameworks with well-designed tool augmentation \citep{schick2023toolformer}, external memory \citep{park2023generative} and better scaffolding \citep{wei2022chain,shinn2023reflexion} to make it more effective -- perception and understanding of the environment still remains a major challenge.

In order to address the above challenges, our work investigates an orthogonal direction to more complex agent architectures and asks -- \emph{Can we replace complex memory and information-gathering processes in agents with a single, long-context model?} Understanding this question has important implications for our understanding of agent design. Although a pure LCLM-based approach is more expensive than a retrieval system, if a single long-context model is competitive with complex scaffolding methods, further improvements in the capability and cost of long-context models may lead to a simpler and more monolithic future. Such a move towards a more monolithic system has significant precedent, mirroring past developments in computer vision \citep{krizhevsky2012imagenet}, statistical machine translation \citep{bahdanau2015neural}, and NLP \citep{brown2020languagemodelsfewshotlearners} where complex and specialized pipelines were replaced by monolithic neural networks.

%We attempt to answer these questions using repository-level software engineering tasks on SWE-Bench-Verified \citep{openaiverified}. 
%{\color{red}Pavan: First big push on agentic with the challenges X, Y, Z, then resolved with non-agentic approaches to just remind us to keep things simple with these advantages, we go further.}

To address our research question, we propose a simplified, scaffolding-free approach that leverages LCLMs' capabilities to solve problems with complete environment state information, minimizing human engineering effort. Our approach treats the LCLM as handling all of perception for the agent, effectively reducing exploration-intensive tasks to a standard prompting one. Overall, this work explores LCLMs for SWE-Bench-Verified \citep{openaiverified} with the following contributions: 

\begin{itemize}[leftmargin=2em]
    \item We show that a simplified agentic method without tools and scaffolding on LCLMs outperforms more complex agentic pipelines by 6\%.

    \item We identify a collection of simple prompting techniques that take an LCLM, specifically Gemini-1.5-Pro based system for SWE-bench from 9\% to 32\%  \tofill{(before patch validation)}. 
    
    \item We show that a further two-stage modification of our LCLM approach that leverages a stronger Claude 3.7 based solver makes this competitive with the state-of-the-art, attaining 49\% solve rate.
    
\end{itemize}


%{\color{red}Pavan: This should be part of the contribution list if its novel. Intro, is more about this work being an investigation of Long Context Models rather than an approach. Might be good to stick to that theory?}

%We find this approach is highly effective, outperforming scaffolding- and agent-based baselines in matched comparisons. However, we still find a gap relative to the strongest agents and retrieval based pipelines today. We identify that this gap is due to the weaker overall capability of LCLMs, and show that a simple hybrid of LCLM and short context LMs largely closes this gap. 

%Our contributions include:

% \begin{itemize}[leftmargin=2em]
%     \item We show that a simplified agentic method without tools and scaffolding on LCLMs outperforms more complex agentic pipelines by 6\%.

%     \item We identify a collection of simple prompting techniques that take an LCLM, specifically Gemini-1.5-Pro based system for SWE-bench from 9\% to 32\%  \tofill{(before patch validation)}. 
    
%     \item We show that a further two-stage modification of our LCLM approach that leverages a stronger Claude 3.7 based solver makes this competitive with the state-of-the-art, attaining 49\% solve rate.
    
% \end{itemize}

% Second paragraph: LMs are excellent at close-ended problem solving (partially due to their pretraining paradigm). One important task, repository-level software engineering, has recently gained significant attention as the emergence of SWE-Bench. There are two mainstream methodology of solving the task: agentic pipeline and non-iterative scaffolding containing multiple steps. Specifically, many methods are proposed to solve it through agentic frameworks, utilizing multi-turn interaction and tools such as file/code searching and shell commands execution, imitating the human software engineers' workflows. Agentless\citep{} pointed out the limitation of those agentic systems lies in complex tool usage, lack of control in planning and limited ability to self-reflect, and proposed a non-agentic scaffold explicitly do prompting-based and retrieval-based localizing, repair candidate proposing and patch validation with tests. They showed they can achieve comparable performance and lower cost. Even though largely simplified, it still requires a carefully human designed multi-step pipeline including file-level, element-level localization, etc. That is, previous works hugely relies on human designed pipeline. 

% While these approaches demonstrate promising results, they share a common limitation: they rely heavily on carefully designed human scaffolding. As observed across domains like traditional NLP and autonomous driving, such handcrafted scaffolds often struggle with end-to-end optimization and domain adaptation challenges. In contrast, more straightforward approaches that scale data and computation have frequently proven superior. The need for sophisticated scaffolding in previous methods stems from the challenge of localization within partially observable environments, where sequential actions must be taken without complete state visibility.




% As shown in many domains like traditional NLP tasks and self-driving, handcrafted scaffold design usually suffers from challenge in end-to-end optimization and  domain adaptation. It turns out more brute-force paradigm with scaling data and computation are usually better solution. Thus, a scaffolding-free configuration need to be carefully considered. The need of the scaffolding in the previous methods design are due to the challenging localization process, which makes people compromise to the unvisible whole state and take sequential actions based on partially observed states. 

% Recent works showed the emergent capability of long-context language models (LCLM), demonstrating the feasibility of retrieval and reasoning given a large context window. Motivated by the discussion above, we should first take a step back and ask the following introspective question: \textit{Can long-context language model directly solve the complex tasks that are previously expected by agentic framework?}




==> tables/ablation_table.tex <==


\begin{table}[ht]
    \centering
        \centering
        \caption{\textbf{Ablation study on key components of our \textsc{DirectSolve} method}. Results are on a random subset of 100 instances from SWE-Bench-Verified.}
\begin{tabular}{@{}l l c c@{}}
\toprule
% \multicolumn{4}{c}{\textbf{Gemini-Pro 1.5 Performance}} \\ \midrule
\textbf{Ablation}       & \textbf{Pass @ 1} & \textbf{Pass @ 8} \\ \midrule
DirectSolve method  &                   32\%   &   50\%  \\ 
~~w/o CoT prompt     &      9\%               & 16\%  \\ 
~~w/o relevant code restatement   &             28\%           &  49\%   \\ 
~~w/o add file index       &          27\%            &  44\% \\ 
~~w/o removing comments and docstrings      &    27\%                  &  41\% \\ 
% w few-shot prompt     &                     &   \\ 
\bottomrule
\end{tabular}
\label{tab:ablation_study}
\end{table}






==> tables/benchmark_models.tex <==

% \begin{table}[t!]
% \centering
% \caption{\textbf{Benchmarking state-of-the-art LCLMs as state-in-context agents with our methods}. The evaluations are conduced on the random subset of 100 instances from SWE-Bench-Verified.}
% \label{tab:benchmarking_results}
% \begin{tabular}{@{}l l c c@{}}
% \toprule
% \textbf{Approach}          & \textbf{Model}                & \textbf{pass@1} & \textbf{pass@8} \\ \midrule
% \onestep                  & Gemini-1.5-Pro       &             32\%        &    50\%  \\
% \onestep              & Gemini-2.0-Pro                &          24\%           &  34\%  \\
% \onestep               & Minimax-Text-001                    &     15\%        &     20\%        \\
% \onestep                     & Gemini-Flash-2.0                &        24\%             &    37\%     \\
% \midrule 
% \twostep                  & Gemini-1.5-Pro       &           34\%          &    48\%  \\
% \twostep             & Gemini-2.0-Pro                &        33\%            &   47\%  \\
% \twostep               & Minimax-Text-001                     &          20\%        &   32\%    \\
% \twostep                     & Gemini-Flash-2.0                &          29\%           &      46\%     \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[t!]
% \centering
% \caption{\textbf{Benchmarking state-of-the-art LCLMs as state-in-context agents with our methods}. Evaluations are conducted on a random subset of 100 instances from SWE-Bench-Verified.}
% \label{tab:benchmarking_results}
% \begin{tabular}{@{}l l c c@{}}
% \toprule
% \textbf{Approach} & \textbf{Model} & \textbf{pass@1} & \textbf{pass@8} \\ \midrule
% \multirow{4}{*}{\onestep} & Gemini-1.5-Pro & 32\% & 50\% \\
%  & Gemini-2.0-Pro & 24\% & 34\% \\
%  & Gemini-Flash-2.0 & 24\% & 37\% \\ 
%  & Minimax-Text-001 & 15\% & 20\% \\
%  \midrule
% \multirow{4}{*}{\twostep} & Gemini-1.5-Pro & 34\% & 48\% \\
%  & Gemini-2.0-Pro & 33\% & 47\% \\
%  & Gemini-Flash-2.0 & 29\% & 46\% \\
%  & Minimax-Text-001 & 20\% & 32\% \\
% \bottomrule
% \end{tabular}
% \end{table}

==> tables/localization_comparison.tex <==
\begin{table}[t!]
  \centering
  \caption{\textbf{File localization error comparison} between the scaffolding-based approach in Agentless and our LCLM-based file selection in \twostep, both using Gemini Pro 1.5. Our LCLM-based file selection not only simplifies the localization procedure but also significantly improves localization accuracy, with more pronounced gains when aggregating selection results over $N=8$ samples with majority voting.}
  \begin{tabular}{lccccc}
    \toprule
    Method & K = 3 &  K = 6 & K = 10 \\
    \midrule
    Agentless prompting-based & 138 & 116 & -- \\
    Agentless embedding-based & 165 & 119 & 102 \\    
    Agentless combined & 135 & 88 & 66 \\
    \midrule
    LCLM one-call & 112  & 75 & 56 \\
    LCLM one-call (N = 8) & 100  & 62 & 47 \\
    \bottomrule
  \end{tabular}
  \label{tab:localization_error}

\end{table}

==> tables/target_file_loc.tex <==
\begin{figure*}[t]
  \centering
  \begin{minipage}[b]{0.45\textwidth}
    \centering
    \begin{tabular}{lccc}
      \toprule
      Metrics & Front & End & Random \\
      \midrule
      pass@1 & 32\%  & 26\% & 28\% \\
      pass@8 & 50\%  & 43\% & 41\% \\
      \bottomrule
    \end{tabular}
    \captionof{table}{Impact of target file location on LCLM DirectSolve performance with 1M token prompts. Higher scores indicate better performance.}
    \label{tab:file-location}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.5\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots/ablation_context_length.png}
    \captionof{figure}{Accuracy vs. Context Length for DirectSolve with target files placed at the front of the prompt. Performance decreases as context length increases for both Self-Consistency and Best-of-8 approaches.}
    \label{fig:context-length}
  \end{minipage}
\end{figure*}
